Prolog Coding Guidelines: Status and Tool Support

The importance of coding guidelines is generally accepted throughout developers of every programming language. Naturally, Prolog makes no exception. However, establishing coding guidelines is fraught with obstacles: Finding common ground on kind and selection of rules is matter of debate; once found, adhering to or enforcing rules is complicated as well, not least because of Prolog's flexible syntax without keywords. In this paper, we evaluate the status of coding guidelines in the Prolog community and discuss to what extent they can be automatically verified. We implemented a linter for Prolog and applied it to several packages to get a hold on the current state of the community.

==> eptcsdata.tex <==
\providecommand{\firstpage}{8}
\providecommand{\publicationstatus}{B. Bogaerts, E. Erdem, P. Fodor, A. Formisano,\\ 
G. Ianni, D. Inclezan, G. Vidal, A. Villanueva, \\
M. De Vos, F. Yang (Eds.): International \\
Conference on Logic Programming 2019 (ICLP'19).\\
EPTCS 306, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.306.8}{10.4204/EPTCS.306.8}}

